TabReD: Analyzing Pitfalls and Filling the Gaps in Tabular Deep Learning Benchmarks

Advances in machine learning research drive progress in real-world applications. To ensure this progress, it is important to understand the potential pitfalls on the way from a novel method's success on academic benchmarks to its practical deployment. In this work, we analyze existing tabular benchmarks and find two common characteristics of tabular data in typical industrial applications that are underrepresented in the datasets usually used for evaluation in the literature. First, in real-world deployment scenarios, distribution of data often changes over time. To account for this distribution drift, time-based train/test splits should be used in evaluation. However, popular tabular datasets often lack timestamp metadata to enable such evaluation. Second, a considerable portion of datasets in production settings stem from extensive data acquisition and feature engineering pipelines. This can have an impact on the absolute and relative number of predictive, uninformative, and correlated features compared to academic datasets. In this work, we aim to understand how recent research advances in tabular deep learning transfer to these underrepresented conditions. To this end, we introduce TabReD -- a collection of eight industry-grade tabular datasets. We reassess a large number of tabular ML models and techniques on TabReD. We demonstrate that evaluation on time-based data splits leads to different methods ranking, compared to evaluation on random splits, which are common in current benchmarks. Furthermore, simple MLP-like architectures and GBDT show the best results on the TabReD datasets, while other methods are less effective in the new setting.

==> data/tab-main-without-bold-ranks.tex <==
\begin{tabular}{lccccccccc}
\toprule
\multirow{3}{*}{Methods} & \multicolumn{3}{c}{Classification {\small (ROC AUC \textuparrow)}} & \multicolumn{5}{c}{Regression {\small (RMSE \textdownarrow)}}  & \multirow{3}{*}{\footnotesize \shortstack{Average \\ Rank}} \\
% \multirow{3}{*}{\footnotesize \shortstack{TabReD \\ Score \\ \tiny Q50 / min / max}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-9}
& \multirow{2}{*}{\footnotesize \shortstack{Homesite \\ Insurance}} & \multirow{2}{*}{\footnotesize \shortstack{Ecom \\ Offers}} & \multirow{2}{*}{\footnotesize \shortstack{HomeCredit \\ Default}} & \multirow{2}{*}{\footnotesize \shortstack{Sberbank \\ Housing}} & \multirow{2}{*}{\footnotesize \shortstack{Cooking \\ Time}} & \multirow{2}{*}{\footnotesize \shortstack{Delivery \\ ETA}} & \multirow{2}{*}{\footnotesize \shortstack{Maps \\ Routing}} & \multirow{2}{*}{\footnotesize Weather}
\\
\\

\midrule
\multicolumn{10}{l}{\hspace{0.1em} \textbf{Classical ML Baselines}} \vspace{4px} \\ 

XGBoost
 & {\footnotesize 0.9601}
 & {\footnotesize 0.5763}
 & \textbf{{\footnotesize 0.8670}}
 & \textbf{{\footnotesize 0.2419}}
 & {\footnotesize 0.4823}
 & \underline{{\footnotesize 0.5468}}
 & \textbf{{\footnotesize 0.1616}}
 & \underline{{\footnotesize 1.4671}}
 & {\footnotesize 2.2 $\pm$ 1.3}\\
LightGBM
 & {\footnotesize 0.9603}
 & {\footnotesize 0.5758}
 & \underline{{\footnotesize 0.8664}}
 & \underline{{\footnotesize 0.2468}}
 & {\footnotesize 0.4826}
 & \underline{{\footnotesize 0.5468}}
 & \underline{{\footnotesize 0.1618}}
 & \textbf{{\footnotesize 1.4625}}
 & {\footnotesize 2.6 $\pm$ 1.2}\\
CatBoost
 & \underline{{\footnotesize 0.9606}}
 & {\footnotesize 0.5596}
 & {\footnotesize 0.8621}
 & \underline{{\footnotesize 0.2482}}
 & {\footnotesize 0.4823}
 & \textbf{{\footnotesize 0.5465}}
 & {\footnotesize 0.1619}
 & \underline{{\footnotesize 1.4688}}
 & {\footnotesize 2.8 $\pm$ 1.4}\\
RandomForest
 & {\footnotesize 0.9570}
 & {\footnotesize 0.5764}
 & {\footnotesize 0.8269}
 & {\footnotesize 0.2640}
 & {\footnotesize 0.4884}
 & {\footnotesize 0.5959}
 & {\footnotesize 0.1653}
 & {\footnotesize 1.5838}
 & {\footnotesize 6.4 $\pm$ 1.7}\\
Linear
 & {\footnotesize 0.9290}
 & {\footnotesize 0.5665}
 & {\footnotesize 0.8168}
 & {\footnotesize 0.2509}
 & {\footnotesize 0.4882}
 & {\footnotesize 0.5579}
 & {\footnotesize 0.1709}
 & {\footnotesize 1.7679}
 & {\footnotesize 7.4 $\pm$ 2.2}\\

\midrule
\multicolumn{10}{l}{\hspace{0.1em} \textbf{Deep Learning Methods}} \vspace{4px} \\ 

MLP
 & {\footnotesize 0.9500}
 & \textbf{{\footnotesize 0.6015}}
 & {\footnotesize 0.8545}
 & {\footnotesize 0.2508}
 & \underline{{\footnotesize 0.4820}}
 & {\footnotesize 0.5504}
 & {\footnotesize 0.1622}
 & {\footnotesize 1.5470}
 & {\footnotesize 3.6 $\pm$ 1.6}\\
SNN
 & {\footnotesize 0.9492}
 & \underline{{\footnotesize 0.5996}}
 & {\footnotesize 0.8551}
 & {\footnotesize 0.2858}
 & {\footnotesize 0.4838}
 & {\footnotesize 0.5544}
 & {\footnotesize 0.1651}
 & {\footnotesize 1.5649}
 & {\footnotesize 5.5 $\pm$ 1.8}\\
DCNv2
 & {\footnotesize 0.9392}
 & {\footnotesize 0.5955}
 & {\footnotesize 0.8466}
 & {\footnotesize 0.2770}
 & {\footnotesize 0.4842}
 & {\footnotesize 0.5532}
 & {\footnotesize 0.1672}
 & {\footnotesize 1.5782}
 & {\footnotesize 6.4 $\pm$ 2.1}\\
ResNet
 & {\footnotesize 0.9469}
 & \underline{{\footnotesize 0.5998}}
 & {\footnotesize 0.8493}
 & {\footnotesize 0.2743}
 & {\footnotesize 0.4825}
 & {\footnotesize 0.5527}
 & {\footnotesize 0.1625}
 & {\footnotesize 1.5021}
 & {\footnotesize 4.6 $\pm$ 1.7}\\
FT-Transformer
 & \textbf{{\footnotesize 0.9622}}
 & {\footnotesize 0.5775}
 & {\footnotesize 0.8571}
 & \underline{{\footnotesize 0.2440}}
 & \underline{{\footnotesize 0.4820}}
 & {\footnotesize 0.5542}
 & {\footnotesize 0.1625}
 & {\footnotesize 1.5104}
 & {\footnotesize 3.5 $\pm$ 1.5}\\
MLP (PLR)
 & \textbf{{\footnotesize 0.9621}}
 & {\footnotesize 0.5957}
 & {\footnotesize 0.8568}
 & \underline{{\footnotesize 0.2438}}
 & \textbf{{\footnotesize 0.4812}}
 & {\footnotesize 0.5527}
 & \textbf{{\footnotesize 0.1616}}
 & {\footnotesize 1.5177}
 & {\footnotesize 2.5 $\pm$ 1.3}\\
TabR
 & {\footnotesize 0.9487}
 & {\footnotesize 0.5943}
 & {\footnotesize 0.8501}
 & {\footnotesize 0.2820}
 & {\footnotesize 0.4828}
 & {\footnotesize 0.5514}
 & {\footnotesize 0.1639}
 & \underline{{\footnotesize 1.4666}}
 & {\footnotesize 4.8 $\pm$ 1.6}\\
TabR (causal)
 & {\footnotesize 0.9522}
 & {\footnotesize 0.5850}
 & {\footnotesize 0.8484}
 & {\footnotesize 0.2851}
 & {\footnotesize 0.4825}
 & {\footnotesize 0.5541}
 & {\footnotesize 0.1637}
 & \textbf{{\footnotesize 1.4622}}
 & {\footnotesize 4.5 $\pm$ 1.5}\\
Trompt
 & {\footnotesize 0.9546}
 & {\footnotesize 0.5792}
 & {\footnotesize 0.8381}
 & {\footnotesize 0.2596}
 & {\footnotesize 0.4834}
 & {\footnotesize 0.5563}
 & {\footnotesize 0.1652}
 & {\footnotesize 1.5722}
 & {\footnotesize 5.9 $\pm$ 1.5}\\

\midrule
\multicolumn{10}{l}{\hspace{0.1em} \textbf{OOD Robustness Methods}} \vspace{4px} \\ 

CORAL
 & {\footnotesize 0.9498}
 & \textbf{{\footnotesize 0.6004}}
 & {\footnotesize 0.8549}
 & {\footnotesize 0.2645}
 & \underline{{\footnotesize 0.4821}}
 & {\footnotesize 0.5498}
 & {\footnotesize 0.1622}
 & {\footnotesize 1.5591}
 & {\footnotesize 3.9 $\pm$ 1.8}\\
DFR
 & {\footnotesize 0.9499}
 & \textbf{{\footnotesize 0.6013}}
 & {\footnotesize 0.8545}
 & {\footnotesize 0.2494}
 & \underline{{\footnotesize 0.4819}}
 & {\footnotesize 0.5515}
 & {\footnotesize 0.1626}
 & {\footnotesize 1.5513}
 & {\footnotesize 4.0 $\pm$ 1.7}\\
% XGBoost & \textbf{0.961}{\footnotesize$\pm$0.0003} & 0.563{\footnotesize$\pm$0.0093} & 0.424{\footnotesize$\pm$0.0008} & 0.486{\footnotesize$\pm$0.0001} & 0.549{\footnotesize$\pm$0.0002} & \textbf{0.161}{\footnotesize$\pm$0.0000} & 1.457{\footnotesize$\pm$0.0006} & 2.4 $\pm$ 1.6 \\
% CatBoost & \textbf{0.961}{\footnotesize$\pm$0.0005} & 0.593{\footnotesize$\pm$0.0031} & 0.428{\footnotesize$\pm$0.0049} & 0.486{\footnotesize$\pm$0.0001} & \textbf{0.548}{\footnotesize$\pm$0.0001} & 0.161{\footnotesize$\pm$0.0000} & 1.463{\footnotesize$\pm$0.0013} & 2.4 $\pm$ 1.0 \\
% LightGBM & \textbf{0.962}{\footnotesize$\pm$0.0007} & 0.600{\footnotesize$\pm$0.0021} & 0.430{\footnotesize$\pm$0.0006} & 0.486{\footnotesize$\pm$0.0001} & 0.549{\footnotesize$\pm$0.0001} & 0.161{\footnotesize$\pm$0.0000} & 1.455{\footnotesize$\pm$0.0008} & 2.1 $\pm$ 0.6 \\
% RandomForest & 0.816{\footnotesize$\pm$0.0007} & 0.514{\footnotesize$\pm$0.0004} & 0.437{\footnotesize$\pm$0.0012} & 0.491{\footnotesize$\pm$0.0000} & 0.558{\footnotesize$\pm$0.0001} & 0.164{\footnotesize$\pm$0.0000} & 1.564{\footnotesize$\pm$0.0001} & 6.9 $\pm$ 1.7 \\
% MLP & 0.950{\footnotesize$\pm$0.0008} & 0.581{\footnotesize$\pm$0.0050} & 0.440{\footnotesize$\pm$0.0134} & 0.487{\footnotesize$\pm$0.0003} & 0.554{\footnotesize$\pm$0.0010} & 0.163{\footnotesize$\pm$0.0001} & 1.520{\footnotesize$\pm$0.0069} & 5.0 $\pm$ 1.5 \\
% SNN & 0.949{\footnotesize$\pm$0.0015} & 0.597{\footnotesize$\pm$0.0065} & 0.455{\footnotesize$\pm$0.0228} & 0.488{\footnotesize$\pm$0.0004} & 0.553{\footnotesize$\pm$0.0008} & 0.163{\footnotesize$\pm$0.0003} & 1.529{\footnotesize$\pm$0.0042} & 5.3 $\pm$ 1.8 \\
% ResNet & 0.945{\footnotesize$\pm$0.0019} & 0.598{\footnotesize$\pm$0.0096} & 0.445{\footnotesize$\pm$0.0157} & 0.487{\footnotesize$\pm$0.0003} & 0.551{\footnotesize$\pm$0.0005} & 0.163{\footnotesize$\pm$0.0002} & 1.477{\footnotesize$\pm$0.0056} & 4.3 $\pm$ 1.3 \\
% DCNv2 & 0.928{\footnotesize$\pm$0.0150} & 0.566{\footnotesize$\pm$0.0331} & 0.447{\footnotesize$\pm$0.0132} & 0.488{\footnotesize$\pm$0.0013} & 0.554{\footnotesize$\pm$0.0025} & 0.164{\footnotesize$\pm$0.0002} & 1.524{\footnotesize$\pm$0.0066} & 6.1 $\pm$ 1.2 \\
% FT-Transformer & 0.950{\footnotesize$\pm$0.0062} & 0.589{\footnotesize$\pm$0.0026} & 0.435{\footnotesize$\pm$0.0066} & \textbf{0.486}{\footnotesize$\pm$0.0005} & 0.556{\footnotesize$\pm$0.0022} & 0.162{\footnotesize$\pm$0.0002} & 1.500{\footnotesize$\pm$0.0079} & 4.0 $\pm$ 1.5 \\
% MLP (PLR) & \textbf{0.961}{\footnotesize$\pm$0.0005} & \textbf{0.607}{\footnotesize$\pm$0.0032} & \textbf{0.421}{\footnotesize$\pm$0.0022} & \textbf{0.485}{\footnotesize$\pm$0.0004} & 0.553{\footnotesize$\pm$0.0012} & 0.161{\footnotesize$\pm$0.0002} & 1.510{\footnotesize$\pm$0.0062} & 2.7 $\pm$ 2.2 \\
% TabR & 0.949{\footnotesize$\pm$0.0029} & 0.594{\footnotesize$\pm$0.0093} & 0.437{\footnotesize$\pm$0.0055} & 0.487{\footnotesize$\pm$0.0005} & 0.556{\footnotesize$\pm$0.0015} & 0.163{\footnotesize$\pm$0.0003} & 1.463{\footnotesize$\pm$0.0039} & 4.4 $\pm$ 1.2 \\
% TabR (causal) & 0.946{\footnotesize$\pm$0.0039} & 0.590{\footnotesize$\pm$0.0081} & 0.445{\footnotesize$\pm$0.0180} & 0.486{\footnotesize$\pm$0.0008} & 0.558{\footnotesize$\pm$0.0025} & 0.163{\footnotesize$\pm$0.0003} & \textbf{1.442}{\footnotesize$\pm$0.0030} & 4.3 $\pm$ 2.0 \\
% Trompt & 0.957{\footnotesize$\pm$0.0023} & 0.590{\footnotesize$\pm$0.0079} & 0.434{\footnotesize$\pm$0.0049} & 0.490{\footnotesize$\pm$0.0034} & 0.557{\footnotesize$\pm$0.0015} & 0.164{\footnotesize$\pm$0.0000} & 1.572{\footnotesize$\pm$0.0504} & 5.9 $\pm$ 2.7 \\
\bottomrule
\end{tabular}


==> data/tabred-datasets-review.tex <==
% Homesite
\subsection*{\href{https://www.kaggle.com/competitions/homesite-quote-conversion/overview}{Homesite Insurance}}

\textbf{Task}: Classification

\textbf{\#Samples}: 260,753 \hspace{10px} \textbf{\#Features}: 299 \hspace{10px} \textbf{Year}: 2015

\textbf{Comments}: This is a dataset from a Kaggle competition hosted by Homesite Insurance \citep{homesite-quote-conversion}. The task is predicting whether a customer will buy a home insurance policy based on user and insurance policy features (user, policy, sales and geographic information). Each row in the dataset corresponds to a potential [customer, policy] pair, the target indicates whether a customer bought the policy. Timeframe from 2013-01-01 to 2015-05-18.


% ECOM
\subsection*{\href{https://www.kaggle.com/competitions/acquire-valued-shoppers-challenge/overview}{Ecom Offers}}

\textbf{Task}: Classification

\textbf{\#Samples}: 160,057 \hspace{10px} \textbf{\#Features}: 119 \hspace{10px} \textbf{Year}: 2014

\textbf{Comments}: This is a dataset from a Kaggle competition hosted by the online book and game retailer DMDave \citep{acquire-valued-shoppers-challenge}. The task in this dataset is a representative example of modeling customer loyalty in e-commerce. Concretely, the task is classifying whether a customer will redeem a discount offer based on features from two months' worth of transaction history. We base our feature engineering on one of the top solutions \citep{ecom-offers-preprocessing}. Timeframe from 2013-03-01 to 2013-04-30.

% Homecredit
\subsection*{\href{https://www.kaggle.com/competitions/home-credit-credit-risk-model-stability}{Homecredit Default}}

\textbf{Task}: Classification

\textbf{\#Samples}: 1,526,659 \hspace{10px} \textbf{\#Samples Used} 381,664 \hspace{10px} \textbf{\#Features}: 696 \hspace{10px} \textbf{Year}: 2024

\textbf{Comments}: This is a second iteration of the popular HomeCredit tabular competition \citep{home-credit-credit-risk-model-stability}. The task is to predict whether bank clients will default on a loan, based on bank internal information and external information like credit bureau and tax registry data. This year competition focus was the model prediction stability over time. Compared to the more popular prior competition, this time there is more data and the timestamps are available.
We base feature engineering and preprocessing code on top solutions \citep{homecredit-preprocessing}. Timeframe from 2019-01-01 to 2020-10-05.


% Sber
\subsection*{\href{https://www.kaggle.com/competitions/sberbank-russian-housing-market}{Sberbank Housing}}

\textbf{Task}: Regression

\textbf{\#Samples}:  28,321 \hspace{10px} \textbf{\#Features}: 392 \hspace{10px} \textbf{Year}: 2017

\textbf{Comments}: This dataset is from a Kaggle competition, hosted by Sberbank \citep{sberbank-russian-housing-market}. This dataset provides information about over 30000 transactions made in the Moscow housing market. The task is to predict the sale price of each property using the provided features describing each property condition, location, and neighborhood, as well as country economic indicators at the moment of the sale. We base our preprocessing code on discussions and solutions from the competition \citep{sberbank-first-place, sberbank-outliers}. Timeframe from 2011-08-20 to 2015-06-30.


% Cooking
\subsection*{\href{https://www.kaggle.com/datasets/pcovkrd84mejm/cooking-time}{Cooking Time}}

\textbf{Task}: Regression

\textbf{\#Samples}: 12,799,642 \hspace{10px} \textbf{\#Samples Used} 319,986 \hspace{10px} \textbf{\#Features}: 192 \hspace{10px} \textbf{Year}: 2024

\textbf{Comments}: For this dataset, the task is to determine how long it will take for a restaurant to prepare an order placed in a food delivery app. Features are constructed based on the information about the order contents and historical information about cooking time for the restaurant and brand, the target is a logarithm of minutes it took to cook the placed order. Timeframe from 2023-11-15 to 2024-01-03.


% delivery
\subsection*{\href{https://www.kaggle.com/datasets/pcovkrd84mejm/delivery-eta}{Delivery ETA}}

\textbf{Task}: Regression

\textbf{\#Samples}: 17,044,043 \hspace{10px} \textbf{\#Samples Used} 416,451 \hspace{10px} \textbf{\#Features}: 223 \hspace{10px} \textbf{Year}: 2024

\textbf{Comments}: For this dataset, the task is to determine the estimated time of arrival of an order from
an online grocery store. Features are constructed based on the courier availability, navigation data
and various aggregations of historical information for different time slices, the target is the logarithm
of minutes it took to deliver an order. Timeframe from 2023-10-20 to 2024-01-25.

% Maps
\subsection*{\href{https://www.kaggle.com/datasets/pcovkrd84mejm/maps-routing}{Maps Routing}}

\textbf{Task}: Regression

\textbf{\#Samples}: 13,639,272  \hspace{10px} \textbf{\#Samples Used} 340,981 \hspace{10px} \textbf{\#Features}: 986 \hspace{10px} \textbf{Year}: 2024

\textbf{Comments}: For this dataset, the task is to predict the travel time in the car navigation system
based on the current road conditions. The features are aggregations of the road graph statistics for the
particular route and various road details (like speed limits). The target is the logarithm of seconds per
kilometre. Timeframe from 2023-11-01 to 2023-12-04.

% Maps
\subsection*{\href{https://www.kaggle.com/datasets/pcovkrd84mejm/tabred-weather}{Weather}}

\textbf{Task}: Regression

\textbf{\#Samples}: 16,951,828  \hspace{10px} \textbf{\#Samples Used} 423,795 \hspace{10px} \textbf{\#Features}: 103 \hspace{10px} \textbf{Year}: 2024

\textbf{Comments}: For this dataset, the task is weather temperature forecasting. This is a dataset similar to the one introduced in \citep{malinin2021weather}, except it is larger, and the time-based split is available and used by default. The features are from weather station measurements and weather forecast physical models. The target is the true temperature for the moment in time. Timeframe from 2022-07-01 to 2023-07-30.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

